Stellar Properties for a Comprehensive Collection of Star Forming Regions in the SDSS APOGEE-2 Survey

The Sloan Digital Sky Survey IV (SDSS-IV) APOGEE-2 primary science goal was to observe red giant stars throughout the Galaxy to study its dynamics, morphology, and chemical evolution. The APOGEE instrument, a high-resolution 300 fiber H-band (1.55-1.71 micron) spectrograph, is also ideal to study other stellar populations in the Galaxy, among which are a number of star forming regions and young open clusters. We present the results of the determination of six stellar properties ($T_{eff}$, $\log{g}$, [Fe/H], $L/L_\odot$, $M/M_\odot$, and ages) for a sample that is composed of 3360 young stars, of sub-solar to super-solar types, in sixteen Galactic star formation and young open cluster regions. Those sources were selected by using a clustering method that removes most of the field contamination. Samples were also refined by removing targets affected by various systematic effects of the parameter determination. The final samples are presented in a comprehensive catalog that includes all six estimated parameters. This overview study also includes parameter spatial distribution maps for all regions and Hertzprung-Russell ($L/L_\odot$ vs. $T_{eff}$) diagrams. This study serves as a guide for detailed studies on individual regions, and paves the way for the future studies on the global properties of stars in the pre-main sequence phase of stellar evolution using more robust samples.

==> Table3.tex <==
\begin{deluxetable}{lccccc}
\tablecaption{Circumstellar Emission per Region\tablenotemark{1} \label{tab:cdstats}}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{Region} & \multicolumn{5}{c}{No. of Sources} \\
\colhead{} & \colhead{Class I} & \colhead{Class II} 
& \colhead{Transitional} & \colhead{EW12\tablenotemark{1}} & \colhead{Br11\tablenotemark{2}} } 
\startdata
$\alpha$-Per  &  0 & 0  &  0 &  0 & 0 \\
California    &  2 & 10 &  0 &  3  & 4\\
Carina        &  0 & 0  &  0 & 49 & 23\\
Corona Aus    & 0 & 1 & 1 & 0 & 0 \\
Cygnus-X      & 5 & 30 & 8 & 18 & 16\\
IC\ 348       &  0 & 26 & 0 & 1 & 7\\
NGC\ 1333     & 0 & 13 & 0 & 2 & 6\\
NGC\ 2264     & 2  & 43 & 4 & 13 & 7\\
$\lambda$-Ori & 0 & 68 & 5 & 5 & 9\\
%Orion\ AB     & 8 & 478 & 22 & 96 \\
Orion\ A     & 3 & 245 & 14 & 79 & 52 \\
Orion\ B     & 1 & 72 & 2 & 24 & 9\\
Orion\ OB1     & 0 & 45 & 5 & 1 & 8\\
Pleiades      & 0  & 0 & 0 & 0 & 0 \\
Rosette       & 9 & 20 & 9 & 5 & 3\\
Taurus        & 0 & 29 & 1 & 1 & 6 \\
Vela          & 0 & 25 & 5 & 13 & -- \\
W3/W4/W5      & 6 & 15 & 1 & 11 & 3 \\
\enddata
\tablenotetext{1}{Number of sources with excess only in WISE bands W1 and W2}
\tablenotetext{2}{Number of sources with accretion indicated by Br11 emission}
\end{deluxetable}

